OpenCity3D: What do Vision-Language Models know about Urban Environments?

Vision-language models (VLMs) show great promise for 3D scene understanding but are mainly applied to indoor spaces or autonomous driving, focusing on low-level tasks like segmentation. This work expands their use to urban-scale environments by leveraging 3D reconstructions from multi-view aerial imagery. We propose OpenCity3D, an approach that addresses high-level tasks, such as population density estimation, building age classification, property price prediction, crime rate assessment, and noise pollution evaluation. Our findings highlight OpenCity3D's impressive zero-shot and few-shot capabilities, showcasing adaptability to new contexts. This research establishes a new paradigm for language-driven urban analytics, enabling applications in planning, policy, and environmental monitoring. See our project page: opencity3d.github.io

==> figures/detroit_prices.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1.0\textwidth]{images/prices-detroit.pdf}
\caption{Zero-shot predicted (left) vs. ground truth (right) prices of sold homes in the Detroit scene. Basemaps are from CartoDB~\cite{cartodb}}
\label{fig:detroit_prices}
\end{figure*}
